HallusionBench: An Advanced Diagnostic Suite for Entangled Language Hallucination and Visual Illusion in Large Vision-Language Models

We introduce HallusionBench, a comprehensive benchmark designed for the evaluation of image-context reasoning. This benchmark presents significant challenges to advanced large visual-language models (LVLMs), such as GPT-4V(Vision), Gemini Pro Vision, Claude 3, and LLaVA-1.5, by emphasizing nuanced understanding and interpretation of visual data. The benchmark comprises 346 images paired with 1129 questions, all meticulously crafted by human experts. We introduce a novel structure for these visual questions designed to establish control groups. This structure enables us to conduct a quantitative analysis of the models' response tendencies, logical consistency, and various failure modes. In our evaluation on HallusionBench, we benchmarked 15 different models, highlighting a 31.42% question-pair accuracy achieved by the state-of-the-art GPT-4V. Notably, all other evaluated models achieve accuracy below 16%. Moreover, our analysis not only highlights the observed failure modes, including language hallucination and visual illusion, but also deepens an understanding of these pitfalls. Our comprehensive case studies within HallusionBench shed light on the challenges of hallucination and illusion in LVLMs. Based on these insights, we suggest potential pathways for their future improvement. The benchmark and codebase can be accessed at https://github.com/tianyi-lab/HallusionBench.

==> format/double_col_format.tex <==
\begin{figure*}
\begin{center}
\begin{tikzpicture}
\node [mybox,title=Illusion Example] (box){%
    \begin{minipage}{\textwidth}


\begin{multicols}{2}
        \bluebold{Prompt: } xxxxx \\[2pt]	
        \begin{subfigure}[b]{0.45\textwidth}
             \centering
             \includegraphics[width = \textwidth]{raw_images/tmp.png}
             % \caption{xxxx}
             % \label{xxxx}
         \end{subfigure}
         \hfill
         \begin{subfigure}[b]{0.45\textwidth}
             \centering
             \includegraphics[width = \textwidth]{raw_images/tmp.png}
             % \caption{xxxx}
             % \label{xxxx}
         \end{subfigure}

        \bluebold{GPT-4V: } xxxx
        
        \columnbreak

        \bluebold{Prompt: } xxxxx \\[2pt]
        \begin{subfigure}[b]{0.45\textwidth}
             \centering
             \includegraphics[width = \textwidth]{raw_images/tmp.png}
             % \caption{xxxx}
             % \label{xxxx}
         \end{subfigure}
         \hfill
         \begin{subfigure}[b]{0.45\textwidth}
             \centering
             \includegraphics[width = \textwidth]{raw_images/tmp.png}
             % \caption{xxxx}
             % \label{xxxx}
         \end{subfigure}

        \bluebold{GPT-4V: } xxxx
        
\end{multicols}

    


    \end{minipage}
};
\end{tikzpicture}%
\caption{xxxxxx}
\label{xxxx}
\end{center}
\end{figure*}

% \begin{figure*}
% \begin{center}
% \begin{tikzpicture}
% \node [mybox,title=Illusion Example] (box){%
%     \begin{minipage}{\textwidth}
%         \bluebold{Prompt: } xxxxx \\[2pt]
%  %        \subfloat{
%  %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
%  %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
% 	% } 		
%         \begin{subfigure}[b]{0.45\textwidth}
%              \centering
%              \includegraphics[width = \textwidth]{fig/tmp.png}
%              % \caption{xxxx}
%              % \label{xxxx}
%          \end{subfigure}
%          \hfill
%          \begin{subfigure}[b]{0.45\textwidth}
%              \centering
%              \includegraphics[width=\textwidth]{fig/tmp.png}
%              % \caption{xxxx}
%              % \label{xxxx}
%          \end{subfigure}

%         \bluebold{GPT-4V: } xxxx

%     \end{minipage}
% };
% \end{tikzpicture}%
% \caption{xxxxxx}
% \label{xxxx}
% \end{center}
% \end{figure*}

==> format/map.tex <==
% \zong{need}
% \begin{figure}
% \begin{center}
% \begin{tikzpicture}
% \node [mybox,title=Image Dependent] (box){%
%     \begin{minipage}{0.50\textwidth}
%         \bluebold{Prompt: } Is New Mexico state larger than Texas state from the map? \\[2pt]
%  %        \subfloat{
%  %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
%  %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
% 	% } 		
%         % \begin{subfigure}[b]{0.45\textwidth}
%         %      \centering
%         %      \includegraphics[width = \textwidth]{raw_images/map1.jpeg}
%         %      \caption{Original}
%         %      % \label{xxxx}
%         %  \end{subfigure}
%          \hfill
%          \begin{subfigure}[b]{0.45\textwidth}
%              \centering
%              \includegraphics[width = \textwidth]{raw_images/map2.png}
%              \caption{With Image Context}
%              % \label{xxxx}
%          \end{subfigure}

%         \bluebold{GPT-4V: } Yes, the right orange circle and the left orange circle appear to be the same size.


%     \end{minipage}
% };
% \end{tikzpicture}%
% \caption{xxxxxx}
% \label{xxxx}
% \end{center}
% \end{figure}

\begin{figure}
\begin{center}
\begin{tikzpicture}
    \node [mybox, title=Image Dependent] (box) {
        \begin{minipage}{0.50\textwidth}
            % Nested tikzpicture for the inner box on the left
            \bluebold{Prompt: } Is New Mexico state larger than Texas state from the map? \\
            \begin{tikzpicture}
                \node [text width=0.45\textwidth, fill=blue!20, rounded corners, minimum height=2.6cm, yshift=2cm] (innerbox) {
                   \bluebold{GPT-4V: } No, New Mexico is not larger than Texas. Texas is the second-largest state in the U.S. by land area, following only Alaska. New Mexico is the fifth-largest state by land area.
                };
                % Caption for the blue box
                % \node [below=0.1cm of innerbox, text width=0.45\textwidth, align=center, font=\small] (innerboxcaption) {
                %     Caption for the blue box
                % };
            \end{tikzpicture}
            \hfill % Space between the inner box and the image
            \begin{subfigure}[b]{0.45\textwidth}
                \centering
                \includegraphics[width=\textwidth]{raw_images/map2.png}
                \caption{With Image Context}
            \end{subfigure}
            \\[2pt]
            
            \bluebold{GPT-4V: } Yes, the right orange circle and the left orange circle appear to be the same size.
        \end{minipage}
    };
\end{tikzpicture}
\caption{xxxxxx}
\label{xxxx}
\end{center}
\end{figure}



==> format/single_col_format.tex <==
\begin{figure}

\begin{center}
\begin{tikzpicture}
\node [mybox,title=Image Supplement] (box){%
    \begin{minipage}{\textwidth}
        \bluebold{Prompt: } Is the right orange circle the same size as the left orange circle? \\[2pt]
 %        \subfloat{
 %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
 %        \includegraphics[width = 0.45\columnwidth]{fig/tmp.png}
	% } 
        \centering
        \begin{subfigure}[b]{0.35\textwidth}
            \centering
             \includegraphics[height = 3cm]{raw_images/id_001_o.pdf}
             \caption{Original}
             % \label{xxxx}
         \end{subfigure}
         \hfill
         \begin{subfigure}[b]{0.55\textwidth}
             \centering
             \includegraphics[height = 3cm]{raw_images/id_001_e.pdf}
             \caption{Negative Image}
             % \label{xxxx}
         \end{subfigure}

        \bluebold{GPT-4V: } No, based on the map you provided, Texas is larger than New Mexico.


    \end{minipage}
};
\end{tikzpicture}%
\caption{xxxxxx}
\label{xxxx}
\end{center}
\end{figure}






==> sections/1s-intro.tex <==
\section{Introduction}


%The integration of vision into LLMs represents a significant step toward the development of Artificial General Intelligence (AGI)~\citep{bubeck2023sparks,touvron2023llama,zeng2022socratic,anas_awadalla_2023_7733589,yang2023mm,liu2023visual,zhu2023minigpt,ye2023mplug,liu2020visual,li2023blip}. While LLMs already possess parametric memory, encoding vast amounts of textual data, the addition of perceptual capabilities allows them to archive visual memories and cross-reference them with text. 

In the contemporary digital era, the convergence of language and vision has introduced a transformative paradigm in artificial intelligence. The integration of large language models (LLMs)~\citep{touvron2023llama,chiang2023vicuna,chen2023alpagasus,zhao2023survey,li2023towards,wei2023larger,Xiao2023LargeLM} with vision systems, giving birth to Large Vision-Language Models (LVLMs)~\citep{bubeck2023sparks,touvron2023llama,zeng2022socratic,anas_awadalla_2023_7733589,yang2023mm,liu2023visual,zhu2023minigpt,ye2023mplug,liu2020visual,li2023blip, liu2020visual,tran2020transform}, has been pivotal in driving monumental progress in image reasoning tasks~\citep{saikh2022scienceqa,hossain2019comprehensive,liu2023documentclip,vinyals2016show,liu2023covid,antol2015vqa,masry2022chartqa}. GPT-4V(ison) and LLaVA-1.5 stand as testaments to this advancement, showcasing unprecedented levels of image understanding and reasoning.

%\tian{How to control parametric and external memory? -- Parametric memory leads to hallucination. }
%This enhancement not only improves the model's accuracy in question-answering tasks by utilizing visual inputs but also gets us closer to a tangible embodied AI and a truly intelligent robot in the real world. Recognizing the primacy of vision in human sensory experiences, a majority of LMM research~\citep{liu2023visual,zhu2023minigpt,ye2023mplug,liu2020visual,li2023blip} is focused on enhancing visual processing. Initial studies either adapt a vision encoder to be compatible with a previously trained LLM or employ a vision-language model to transform visual data into textual descriptions for LLM comprehension. \tian{Simplify this paragraph and mention illusion}

%In multi-modality models, perception by the vision module and parametric memory of the LLM are more deeply entangled than previously believed.
%Although GPT-4V(Vision)~\citep{yang2023dawn} and current Large Multimodal Models(LMMs) claim unprecedented visual understanding performance and language creativity, \citep{li2023evaluating,liu2023aligning,zhang2023siren} observed that \textit{current LMMs suffer from severe hallucination issues on input images and output text}. We raise two hypotheses: (i) \textit{ Given the visual input, it's challenging for LMMs to decide whether to generate answers based on their parametric memory or real visual context.} (2) \textit{The vision perception ability of LMMs is still not strong enough to analyze the detailed information.} With the added visual capability of those large models, it is vital to pause and understand the shortcomings of these current models, focusing on targeted improvements rather than blindly stacking parameters and features or expanding the size of the training dataset.



While LVLMs have showcased immense capabilities, they are not without their vulnerabilities. The potent language bias inherent in these state-of-the-art LVLMs can sometimes overshadow the visual context, leading them to rely excessively on language priors, even when they conflict with the image's context \citep{li2023evaluating,liu2023aligning,zhang2023siren,zhai2023investigating}. This dominance of the language component in decision-making can be termed as ``\textit{\textbf{Language Hallucination}}.'' On the other end of the spectrum, the vision modules within these LVLMs, although integral, have shown to be weaker in comparison to their language counterparts. This imbalance can lead to ``\textit{\textbf{Visual Illusion}}'' where erroneous visual interpretations are confidently asserted by the LLMs. To be specific, ``\textit{\textbf{Language Hallucination}}'' \textit{is a perception not based on sensory input, whereas} ``\textit{\textbf{Visual Illusion}}'' \textit{is a misinterpretation of a correct sensory input}. 




%\textit{it's still unclear whether its ability comes from the knowledge of LLM, or it has learned to infer and retrieve similar visual patterns in the large training set \tian{Remove -- bring parametric memory v.s. context}, or it actually possesses the ability to reason across images and text. \tian{Ask questions that we have an answer to.}} With the added visual capability of those large models, it is vital to pause and understand the shortcomings of these current models well, focusing on targeted improvements rather than blindly stacking parameters and features or expanding the size of the training dataset.

Recognizing the importance of understanding and mitigating these challenges, we introduce \ours{}, which is meticulously curated to dive deep into the intricacies of image-context reasoning. We also delve into the recently released GPT-4V(ision)~\citep{yang2023dawn} and LLaVA-1.5~\citep{liu2023improved} and investigate their visual understanding capability. Our analysis of \ours{} offers a granular view of where and how LVLMs stumble, be it through \textit{Visual Illusion} or \textit{Language Hallucination}. This detailed exploration not only illuminates the current shortcomings but also paves the way for future enhancements, ensuring that the next generation of LVLMs is more robust, balanced, and accurate.

The main contributions of this paper are as follows:

%\tian{Points: We asked conflicting questions that contradic common sense or parametric knowledge, which has not been done in other benchmarks? Encourage better reasoning instead of memorizing and repeating. To be a critical thinker.}
\begin{enumerate}
    \item We introduce \ours{}, the first benchmark focusing on the visual illusion and knowledge hallucination of VLMs. 
    % by visual manipulations. 
    \ours{} consists of approximately 200 visual question-answer (QA) pairs, nearly half of which are generated by human experts. The images associated with those QA pairs include unedited images like illusions, charts, maps, posters, videos, and hand-crafted or edited images, spanning topics including math, counting, culture, cartoons, sports, geography, and more.
    \item We explore \ours{} and provide a detailed in-depth analysis of examples on which the SOTA LVLMs such as GPT-4V and LLaVA-1.5 fail. Our analysis attributes the failures to two main factors: \textit{\textbf{Language Hallucination}} and \textit{\textbf{Visual Illusion}}. While the former is caused by the reasoning bias from the parametric memory of LLMs in those models, the latter is due to the misinterpretation of the visual patterns in the image context. 
    % in two major categories -- \textit{\textbf{Visual Dependent}} and \textit{\textbf{Visual Supplement}} -- and several subcategories. 
    % We choose the recently released state-of-the-art LMMs, GPT-4V(Vision) and LLaVA-1.5, as a demonstration of what kind of current vision capabilities the LMMs are lacking and potential explanations and insights. Through those examples, we show how \ours{} can serve as a challenging benchmark for visual reasoning and the issue of hallucination.

    % \item We benchmark a wide range of both closed and open-source VLMs on our proposed \ours{} and show quantitative evaluations. We discover that most of those methods struggle with \ours{} due to poor visual reasoning and hallucination.

\end{enumerate}



% Specifically, we are the first to introduce \ours{} evaluating the knowledge hallucination of LMMs by visual manipulations. \ours{} consists of approximately 200 visual question-answers pairs and 100 manipulated images generated by human experts. 
% \ours{}'s images span diverse types, including natural, illusions, charts, maps, posters, videos, and hand-crafted images, different topics including math, counting, culture, cartoon, sports, geography, sports, and so on. 
% More importantly, our instances can be divided into two big taxonomies: \textit{Visual Dependent} and \textit{Visual Supplement} and several subcategories. Our evaluation strategy is to ask the same question for both the original images and the manipulated image. We will then compare the differences between the answers.


This is still an early report and a work in progress. We will release \ours{} and benchmark it on a wide range of closed and open-source LVLMs.

==> sections/4s-analysis.tex <==
\section{Analysis on \ours{} with GPT-4V and LLaVA-1.5}

In this section, we investigate the vision capability of GPT-4V~\citep{yang2023dawn} and LLaVA-1.5~\citep{liu2023improved} on our proposed \ours{}. \ours{} consists of around 200 visual question-answer pairs, including manipulated images generated by human experts. \ours{}'s images span diverse types (including \textit{\textbf{unedited images like illusions, charts, maps, posters, videos, and hand-crafted images}}) and different topics (including \textit{\textbf{math, counting, culture, cartoon, sports, geography, and so on}}). 
% Our evaluation strategy is to ask the same question with different image inputs. 

In the following sections, we first define the two categories of visual questions in \ours{}, \textit{\textbf{Visual Dependent}} and \textit{\textbf{Visual Supplement}}, and discuss how we design our control group for experimentation. Then, we discuss the two major factors that might lead to incorrect responses: \textit{\textbf{Visual Illusion}} and \textit{\textbf{Language Hallucination}}. Finally, in each of the major categories, we show failed examples from different subcategories with corresponding detailed analyses.

% \subsection{Taxonomies and Control Groups}
\subsection{Taxonomies of Visual Question Types and Control Groups}

% For visual questions, we divide them into two main taxonomies: \textit{\textbf{Visual Dependent}} and \textit{\textbf{Visual Supplement}}.


\subsubsection{Definition of Visual Dependent}

\textbf{\textit{``Visual Dependent''}} questions are defined as \textbf{\textit{questions that do not have an affirmative answer without the visual context.}} Such a question asks about the image itself or something within the image. For example, in Fig.\ref{visual_depend1}, there is no clear answer to the question \textit{"Is the right orange circle the same size as the left orange circle?"} without given images.

% \textit{"Visual Dependent"} means GPT-4V is unable to answer the questions without the visual input. For example, in Fig.\ref{visual_depend2}, GPT-4V can not answer \textit{"Is the right orange circle the same size as the left orange circle?"} without given images. 


\noindent\textbf{{Goal}:} Under this setting, our benchmark is designed to evaluate visual commonsense knowledge and visual reasoning skills. Our exploration and dataset construction are guided by the following questions:

\begin{enumerate}
    \item \textit{How good is the visual understanding and reasoning skill of the model?}
    \item \textit{How does the parametric memory affect the response?}
    %\item \textit{Does the issue of illusion/hallucination also exist in the visual component?}
    \item \textit{Is the model able to capture the temporal relation of multiple images?}
\end{enumerate}

% Our purpose is to evaluate visual commonsense knowledge and visual reasoning skills. 


\noindent\textbf{\textit{Control Group}:} We design the control groups for analysis by asking the same question on both the original image from the Internet as well as the edited image based on the original one. We only modify a small portion of the original image, which would convey different meanings and subsequently affect the correctness of the original answer. We refer to those edited images as \textit{Hard Negative Examples}. 

% In practice, we ask the same questions for the positive(original) images and Hard negative(Edited) images. "Hard negative images" means that we only manipulate small parts of the images, but the semantic meaning becomes the opposite. 



\subsubsection{Definition of Visual Supplement}

\textbf{\textit{``Visual Supplement''}} questions are \textbf{\textit{questions that can be answered without the visual input; the visual component merely provides supplemental information.}} For example, in Fig.\ref{visual_supple4}, GPT-4V can answer \textit{"Is New Mexico state larger than Texas state?"} without the image. Our purpose is to evaluate whether GPT-4V and LLaVA-1.5 can answer the questions based on the images instead of their parametric memory. 
% In practice, we ask the same questions for GPT-4V with or without images.


\noindent\textbf{\textit{Goal}:} Under this setting, our benchmark is designed to evaluate visual reasoning ability and the balance between parametric memory and image context. Our exploration and dataset construction under this category are guided by the following questions:

\begin{enumerate}
    \item \textit{When the model does not know the answer from parametric memory, would the model (still) hallucinate about the images?}
    \item \textit{When the model knows the answers from the parametric memory, would the model get additional details from the visual supplement to answer the question better (especially where there is conflicting information between the two or the parametric memory is out of date)?}
    %\item \textit{Can the model get additional details from the visual supplement to answer the question better?}
    %\item \textit{How would the model handle the trade-off between parametric memory and immediate visual context, especially where there is conflicting information between the two?}
    \item \textit{How well can the model take a visual with dense information (i.e., a graph, chart, map, etc.) and use it for question answering? What manipulation can disturb information extraction?}
\end{enumerate}


\noindent\textbf{\textit{Control Group}:} We design the control groups for analysis by asking the same question with and without images as supplemental information. The supplemental visual context will provide more details that can help to answer the questions, which may conflict with information in the real world.



\subsection{Taxonomies of Failure Types}

We analyze the incorrect answers and categorize the causes into two major types: \textit{\textbf{Visual Illusion}} and \textit{\textbf{Language Hallucination}}.

\textbf{Visual Illusion.} Visual illusion comes from the failure of visual recognition and understanding of the input image. The model could not obtain accurate information or reason about the image correctly.

% \textbf{Parametric Memory Over-fitting.}
% trade-off

\textbf{Language Hallucination.} In Language Hallucination, the model makes false prior assumptions about the input and image context based on its parametric memory. The model should respond based on how the question is framed instead of ignoring it or making false assumptions about the image.



\subsection{Visual Dependent Examples}


From the famous illusions in Fig.\ref{visual_depend1}, Fig.\ref{visual_depend2}, and Fig.\ref{visual_depend3}, we found \textbf{GPT-4V is more knowledgeable than LLaVA-1.5} in recognizing all the illusion cases and knowing their names. However, GPT-4V fails to answer the question faithfully based on the edited images. The reason behind this might be that \textbf{GPT-4V tends to generate answers based on its parametric memory instead of analyzing the images}. Compared to GPT-4V, LLaVA-1.5 performs badly on both the original image and edited images, indicating that \textbf{the visual perception skill of LLaVA-1.5 is limited}. 

From the examples in Fig.\ref{visual_depend4} and Fig.\ref{visual_depend5}, we found both GPT-4V and LLaVA-1.5 are unable to correctly recognize parallel lines, regular triangles, polygons, and other math theorems, meaning that \textbf{geometry and math are still a challenging task for GPT-4V}. 

We further explore GPT-4V's and LLaVA-1.5's abilities in Optical Character Recognition in Fig.\ref{visual_depend6} and Figure Recognition in Fig.\ref{visual_depend7}. From our observations, we found that GPT-4V and LLaVA-1.5 are easily misled by editing the characters in the images, demonstrating that GPT-4V and LLaVA-1.5 generate answers based on their parametric memory instead of visual reasoning. This is because the difference between the original images and edited images is obvious. 

Inspired by~\cite{yang2023dawn}, which shows the promising video understanding of GPT-4V, we also investigate more examples in Fig.\ref{visual_depend_video1} and Fig.\ref{visual_depend_video2}, including several frame sequence examples. The positive sequence and reversed sequence have the opposite semantic meaning, such as \textit{"disappear or appear" and "park or leave"} in Fig.\ref{visual_depend_video1}. From the comparison, we found that \textbf{GPT-4V is unable to distinguish between the positive sequence and the reversed sequence of the images, indicating that there is still much room to improve the video reasoning ability}.




\subsection{Visual Supplement Examples}
In Fig.\ref{visual_supple1}, Fig.\ref{visual_supple2}, and Fig.\ref{visual_supple3}, GPT-4V does not have an affirmative answer if no images are given. Given the image context, GPT-4V and LLaVA-1.5 are unable to understand the chart correctly, indicating that \textbf{their chart reasoning ability is still limited}. In the second example (bottom) of Fig.\ref{visual_supple10}, the predictions of GPT-4V changed completely after we rotated the chart.
% , which also supports this conclusion. 

In Fig.\ref{visual_supple4}, 
% Fig.\ref{visual_supple5}, 
Fig.\ref{visual_supple6}, Fig.\ref{visual_supple8}, Fig.\ref{visual_supple9}, and Fig.\ref{visual_supple10}, GPT-4V and LLaVA-1.5 have an affirmative answer if no images are given. After providing the image, including charts, tables, or maps, we found that they prefer to answer the questions with their knowledge instead of analyzing the image. This might be because \textbf{GPT-4V and LLaVA-1.5 demonstrate a marked dependence on textual reasoning capabilities, often prioritizing them over visual reasoning}. 

From Fig. \ref{visual_supple6} and Fig.\ref{visual_supple7}, we found the knowledge from LLaVA-1.5 is not accurate since it states "\textit{$\pi$ doesn't range from 3.1415926 and 3.1415927}" and "\textit{North Carolina is farther north than Delaware}." This observation also supports our claim that \textbf{GPT-4V is more knowledgeable than LLaVA-1.5}.




==> sections/7-conclusion.tex <==
\section{Conclusion}

In this report, we delve into various examples and failure cases associated with GPT-4V and LLaVA-1.5. Through a detailed examination of these instances, we would like to offer our observations and key insights for future studies:

% Our primary findings are as follows:
\begin{enumerate}
    \item When GPT-4V and LLaVA-1.5 have prior knowledge of the questions in \ours{}, they usually suffer from \textit{\textbf{Language Hallucination}}, and tend to prioritize the prior knowledge and give incorrect answers for over \textit{\textbf{90\%}} of the questions we analyze. \textit{The model should handle the trade-off between parametric memory and context.}
    \item When the GPT-4V and LLaVA-1.5 haven't had the parametric memory or prior knowledge regarding the questions in \ours{}, they can still be prone to \textit{\textbf{Visual Illusion}} and prefer to produce wrong answers about given \textit{\textbf{Geometry\&Math Images, Videos(Multiple Images), Complex Charts and so on}}. \textit{The visual capability of existing VLMs is still limited.}
    \item GPT-4V and LLaVA-1.5 can be easily misled by simple image manipulations in \ours{}, including \textbf{\textit{image flipping, order reversing, masking, optical character editing, object editing, and color editing}}. \textit{The existing VLMs could not handle these manipulations.}
    \item Even with multiple-images support, GPT-4V is unable to capture the temporal relations of multiple images and \textit{\textbf{fails to answer temporal reasoning questions} in \ours{}}. \textit{Those models lack true temporal reasoning ability.}
    \item LLaVA-1.5 performs to be less knowledgeable than GPT-4V and sometimes make commonsense errors in \ours{}.
\end{enumerate}


Based on our observations with those SOTA VLMs and the challenges identified, we introduce \ours{}, which focuses on benchmarking VLMs on those challenging cases in which \textit{\textbf{Language Hallucination}} and/or \textit{\textbf{Visual Illusion}} can easily lead to their failures. We are still expanding our database and will make \ours{} publicly available soon at \href{https://github.com/tianyi-lab/HallusionBench}{https://github.com/tianyi-lab/HallusionBench}.

\section{Acknowledgements}
This work is supported in part by the US Defense Advanced Research Projects Agency (DARPA) Semantic Forensics (SemaFor) Program under HR001120C0124. Any opinions,
findings, and conclusions or recommendations expressed in
this material are those of the authors and do not necessarily reflect the views of the DARPA. We also thank the anonymous reviewers for their constructive feedback.


==> tables/data_distribution.tex <==
% \begin{table}
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{ccccccc}
% \hline
%                                                   &                                       & \textbf{without visual} & \textbf{with original visual} & \textbf{with edited visual} & \multicolumn{2}{c}{\textbf{overall}}            \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{VS}}} & \multicolumn{1}{c|}{\textbf{chart}}   & 76                      & 68                            & \multicolumn{1}{c|}{62}     & \multicolumn{1}{c|}{206} & \multirow{4}{*}{538} \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{table}}   & 43                      & 43                            & \multicolumn{1}{c|}{69}     & \multicolumn{1}{c|}{155} &                      \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{map}}     & 32                      & 32                            & \multicolumn{1}{c|}{32}     & \multicolumn{1}{c|}{96}  &                      \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{ocr}}     & 27                      & 27                            & \multicolumn{1}{c|}{27}     & \multicolumn{1}{c|}{81}  &                      \\ \hline
% \multicolumn{1}{c|}{\multirow{5}{*}{\textbf{VD}}} & \multicolumn{1}{c|}{\textbf{ilusion}} & N/A                     & 72                            & \multicolumn{1}{c|}{72}     & \multicolumn{1}{c|}{144} & \multirow{5}{*}{591} \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{math}}    & N/A                     & 54                            & \multicolumn{1}{c|}{54}     & \multicolumn{1}{c|}{108} &                      \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{others}}  & N/A                     & 39                            & \multicolumn{1}{c|}{41}     & \multicolumn{1}{c|}{80}  &                      \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{video}}   & N/A                     & 69                            & \multicolumn{1}{c|}{101}    & \multicolumn{1}{c|}{170} &                      \\
% \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{poster}}     & N/A                     & 43                            & \multicolumn{1}{c|}{46}     & \multicolumn{1}{c|}{89}  &                      \\ \hline
% \multicolumn{2}{c}{\textbf{overall}}                                                      & 178                     & 447                           & 504                         & \multicolumn{2}{c}{1129}                        \\ \hline
% \end{tabular}
% }
% \caption{Key statistics of HallusionBench.}
% \label{tab:statistics_num}
% \end{table}



% \begin{table}
% \centering
% \setlength{\tabcolsep}{5pt} % Adjust horizontal spacing
% \renewcommand{\arraystretch}{1.2} % Adjust vertical spacing
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c | l|c|c|c|c|c|}
% \hline
% & & \thead{Without\\Visual} & \thead{With\\Original Visual} & \thead{With\\Edited Visual} & \multicolumn{2}{c|}{\textbf{Overall}} \\
% \hline
% \multirow{4}{*}{\textbf{VS}} & \textbf{Chart}   & 76  & 68  & 62  & 206 & \multirow{4}{*}{538} \\
%                              & \textbf{Table}   & 43  & 43  & 69  & 155 & \\
%                              & \textbf{Map}     & 32  & 32  & 32  & 96  & \\
%                              & \textbf{OCR}     & 27  & 27  & 27  & 81  & \\
% \hline
% \multirow{5}{*}{\textbf{VD}} & \textbf{Illusion} & N/A & 72  & 72  & 144 & \multirow{5}{*}{591} \\
%                              & \textbf{Math}    & N/A & 54  & 54  & 108 & \\
%                              & \textbf{Video}   & N/A & 69  & 101 & 170 & \\
%                              & \textbf{Poster}  & N/A & 43  & 46  & 89  & \\
%                              & \textbf{Others}  & N/A & 39  & 41  & 80  & \\
% \hline
% \multicolumn{2}{|c|}{\textbf{Overall}} & 178 & 447 & 504 & \multicolumn{2}{c|}{1129} \\
% \hline
% \end{tabular}
% }
% \caption{Key statistics of HallusionBench.}
% \label{tab:statistics_num}
% \end{table}


\begin{table}
\centering
\setlength{\tabcolsep}{5pt} % Adjust horizontal spacing
\renewcommand{\arraystretch}{1.2} % Adjust vertical spacing
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c | l|c|c|c|c|c}
\hline
& & \thead{Without\\Visual} & \thead{With\\Original Visual} & \thead{With\\Edited Visual} & \multicolumn{2}{c}{\textbf{Overall}} \\
\hline
\multirow{4}{*}{\textbf{VS}} & \textbf{Chart}   & 76  & 68  & 62  & 206 & \multirow{4}{*}{538} \\
                             & \textbf{Table}   & 43  & 43  & 69  & 155 & \\
                             & \textbf{Map}     & 32  & 32  & 32  & 96  & \\
                             & \textbf{OCR}     & 27  & 27  & 27  & 81  & \\
\hline
\multirow{5}{*}{\textbf{VD}} & \textbf{Illusion} & N/A & 72  & 72  & 144 & \multirow{5}{*}{591} \\
                             & \textbf{Math}    & N/A & 54  & 54  & 108 & \\
                             & \textbf{Video}   & N/A & 69  & 101 & 170 & \\
                             & \textbf{Poster}  & N/A & 43  & 46  & 89  & \\
                             & \textbf{Others}  & N/A & 39  & 41  & 80  & \\
\hline
\multicolumn{2}{c|}{\textbf{Overall}} & 178 & 447 & 504 & \multicolumn{2}{c}{1129} \\
\hline
\end{tabular}
}
\caption{Key statistics of HallusionBench.}
\label{tab:statistics_num}
\end{table}


==> tables/leaderboard.tex <==
\begin{table*}[t]
\vspace{-1em}
\caption{\textbf{leaderboard}}
  \label{tab:leaderboard}
  \begin{center}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lcccccccccccccc}
    \toprule
    &  \multicolumn{5}{c}{\textbf{Accuracy}} &  \multicolumn{8}{c}{\textbf{Test}}  \\ \cmidrule(lr){2-6} \cmidrule(lr){7-14}              
    \textbf{Model} & {
    \begin{tabular}{c}
        \textbf{question pair} \\ (qAcc)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{figure} \\ (fAcc)\\
    \end{tabular}
    }
     & {
    \begin{tabular}{c}
        \textbf{easy question} \\ (easy acc)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{hard question} \\ (hard acc)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{question} \\ (acc)\\
    \end{tabular}
    } 
    & {
    \begin{tabular}{c}
        \textbf{Yes/No Bias} \\ (Pct Diff)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{Yes/No Bias} \\ (FP Ratio)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{Consistency Test} \\ (correct)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{Consistency Test} \\ (inconsistent)\\
    \end{tabular}
    }
    & {
    \begin{tabular}{c}
        \textbf{Consistency Test} \\ (wrong)\\
    \end{tabular}
    }
    & \textbf{LH} & \textbf{VI} & \textbf{mixed} \\
    \midrule
    \multicolumn{1}{l}{GPT4V-}   & & & & & & & & & & & &  &      \\
  \bottomrule
\end{tabular}
}
\end{center}
\vspace{-3em}
\end{table*}
